Vision Transformer Based Video Hashing Retrieval for Tracing the Source of Fake Videos

In recent years, the spread of fake videos has brought great influence on individuals and even countries. It is important to provide robust and reliable results for fake videos. The results of conventional detection methods are not reliable and not robust for unseen videos. Another alternative and more effective way is to find the original video of the fake video. For example, fake videos from the Russia-Ukraine war and the Hong Kong law revision storm are refuted by finding the original video. We use an improved retrieval method to find the original video, named ViTHash. Specifically, tracing the source of fake videos requires finding the unique one, which is difficult when there are only small differences in the original videos. To solve the above problems, we designed a novel loss Hash Triplet Loss. In addition, we designed a tool called Localizator to compare the difference between the original traced video and the fake video. We have done extensive experiments on FaceForensics++, Celeb-DF and DeepFakeDetection, and we also have done additional experiments on our built three datasets: DAVIS2016-TL (video inpainting), VSTL (video splicing) and DFTL (similar videos). Experiments have shown that our performance is better than state-of-the-art methods, especially in cross-dataset mode. Experiments also demonstrated that ViTHash is effective in various forgery detection: video inpainting, video splicing and deepfakes. Our code and datasets have been released on GitHub: \url{https://github.com/lajlksdf/vtl}.

==> sec/biography.tex <==
\newpage

\section{Biography Section}
If you have an EPS/PDF photo (graphicx package needed), extra braces are
 needed around the contents of the optional argument to biography to prevent
 the LaTeX parser from getting confused when it sees the complicated
 $\backslash${\tt{includegraphics}} command within an optional argument. (You can create
 your own custom macro containing the $\backslash${\tt{includegraphics}} command to make things
 simpler here.)
 
\vspace{11pt}

\bf{If you include a photo:}\vspace{-33pt}
\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{fig1}}]{Michael Shell}
Use $\backslash${\tt{begin\{IEEEbiography\}}} and then for the 1st argument use $\backslash${\tt{includegraphics}} to declare and link the author photo.
Use the author name as the 3rd argument followed by the biography text.
\end{IEEEbiography}

\vspace{11pt}

\bf{If you will not include a photo:}\vspace{-33pt}
\begin{IEEEbiographynophoto}{John Doe}
Use $\backslash${\tt{begin\{IEEEbiographynophoto\}}} and the author name as the argument followed by the biography text.
\end{IEEEbiographynophoto}




\vfill

==> tbl/Inter-Intra.tex <==

\begin{algorithm}
\caption{Loss functions of \textbf{Hash Triplet Loss}}
\label{algo:inter-intra}
\SetKwInput{KwInput}{Input}
\SetKwInput{KwOutput}{Output}
\DontPrintSemicolon
  
  \KwInput{Triplet hash codes as $\mathbb{H}$\;\hspace{.9cm} Voted hash center as $\vec{o}$}

  \SetKwFunction{FInterLoss}{InterLoss}
  \SetKwFunction{FIntraLoss}{IntraLoss}
  \BlankLine

  
\emph{Calculate the distance between the triplet and the voted hash center}\;
  \SetKwProg{Fn}{Def}{:}{}
  \Fn{\FIntraLoss{$\mathbb{H}$, $\vec{o}$}}{
    intraLoss = 0 \;
    \For{$i$ \KwTo $3$}{
        $\vec{t}$ = $\mathbb{H}$[i]\;
        loss = mean($\vec{t}-\vec{o}$)\;
        intraLoss += loss\;
    }
    \KwRet intraLoss\;
  }
  \;
  
\emph{Calculate the distance between the triplet and the other hash center}\;
  \SetKwProg{Fn}{Def}{:}{}
  \Fn{\FInterLoss{$\mathbb{H}$, $\vec{o}$}}{
    interLoss = 0 \;
    \For{$i$ \KwTo $3$}{
        $\vec{t}$ = $\mathbb{H}$[i]\;
        loss = mean($\vec{t}-\vec{o})$\;
        interLoss += 1 - loss\;
    }
    \KwRet interLoss\;
  }
  \;

\end{algorithm}


==> tex/db-davis.tex <==
\begin{figure}[h]
    \center
    \includegraphics[width=.6\linewidth]{fig/inpainting.jpg}
    \caption{
        DAVIS2016-TL: DAVIS2016-TL is based on the DAVIS2016 dataset and related masks. Using five state-of-the-art objects inpainting methods to synthetic 300 fake videos.
    }
    \label{fig:db_Davis2016}
\end{figure}


==> tex/db-dftl.tex <==
\begin{figure}[ht]
    \center
    \includegraphics[width=.6\linewidth]{fig/human.jpg}
    \caption{
        DFTL:We paid for 75 Asians and each one shot three videos for 15 minutes. We used three Deepfake methods to make fake videos and finally selected some high-quality videos.
    }
    \label{fig:db_DFTL}
\end{figure}


==> tex/db-vstl.tex <==
\begin{figure}[ht]
    \center
    \includegraphics[width=.6\linewidth]{fig/splicing.jpg}
    \caption{
        VSTL: We have carefully manufactured 30 video object splicing videos, many of which are military scenes. The foreground and objects of the video are added frame by frame, and the added object size and position is reasonable.
    }
    \label{fig:db_VSTL}
\end{figure}


==> tex/err.tex <==
 \begin{figure}[ht]
    \centering
      \includegraphics[width=1\linewidth]{fig/err.pdf} 
    \caption{Some tracing errors on different backgrounds and shapes.}
    \label{fig:error}
  \end{figure}

==> tex/similar.tex <==
\begin{figure*}[ht]
    \subfloat[Similar scenes]
    {
        \label{fig:Similar-a}
        \includegraphics[width=.29\textwidth]{fig/similar-a.pdf}
    }
    \subfloat[Same scenes]
    {
        \label{fig:Similar-b}
        \includegraphics[width=.29\textwidth]{fig/similar-b.pdf}
    }
    \subfloat[Error Analysis]
    {
        \label{fig:error}
        \includegraphics[width=.34\textwidth]{fig/err.pdf}
    }\\
    \caption{
        Analysis of the tracing results. (a) These videos are taken by the same person in a similar background. These scenes have different lights and somewhat different backgrounds. (b) These videos are shot by the same person in the same scene, similar to a news conference. These videos are taken from different angles, and the characters' clothes and costumes are the same. (c) These videos have very similar or the same background, only with different face areas.
    }
    \label{fig:Similar}
\end{figure*}

==> tex/trace-result.tex <==
\begin{figure*}[htbp]
\centering
\subfloat[FaceForensics++]
{
\label{fig:FaceForensics}
\includegraphics[width=.2\textwidth]{fig/FF++.pdf}
}
\subfloat[DeepFakeDetection]
{
\label{fig:DeepFakeDetection}
\includegraphics[width=.2\textwidth]{fig/DFD.pdf}
}
\subfloat[VSTL]
{
\label{fig:VSTL}
\includegraphics[width=.2\textwidth]{fig/VSTL.pdf}
}
\subfloat[DAVIS2016-TL]
{
\label{fig:DAVIS2016}
\includegraphics[width=.2\textwidth]{fig/Davis2016.pdf}
}\\
\caption{The tracing results on four datasets: FaceForensics++, DFDC, VSTL and DAVIS2016-TL.}
\label{fig:Retrieval}
\end{figure*}

